Transient narrow high-velocity absorptions in the stationary spectra of SS433

We report on the discovery of rare emergence (31 nights from 360 nights of observations) of narrow absorption features in hydrogen and helium lines in stationary SS433 spectra with velocities ranging from $-650$ to $-1900$ km/s. The components arise independently of the appearance of P-Cygni line profiles which are frequently observed in the SS433 stationary spectra with terminal velocities ranging from $-200$ to $\sim -2500$ km/s. The characteristic rising time of the transient absorptions is about one day and the decay time is about two days. The phenomenology of the absorptions suggests their origin due to hydrodynamic instabilities of wind outflows from a supercritical accretion disk in SS433.

==> journals.tex <==
\newcommand{\aj}{Astronomical Journal}
\newcommand{\actaa}{Acta Astronomica}
\newcommand{\araa}{Annual Review of Astron and Astrophys}
\newcommand{\apj}{Astrophysical Journal}
\newcommand{\apjl}{Astrophysical Journal, Letters}
\newcommand{\apjs}{Astrophysical Journal, Supplement}
\newcommand{\ao}{Applied Optics}
\newcommand{\apss}{Astrophysics and Space Science}
\newcommand{\aap}{Astronomy and Astrophysics}
\newcommand{\aapr}{Astronomy and Astrophysics Reviews}
\newcommand{\aaps}{Astronomy and Astrophysics, Supplement}
\newcommand{\azh}{Astronomicheskii Zhurnal}
\newcommand{\baas}{Bulletin of the AAS}
\newcommand{\caa}{Chinese Astronomy and Astrophysics}
\newcommand{\cjaa}{Chinese Journal of Astronomy and Astrophysics}
\newcommand{\icarus}{Icarus}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\jrasc}{Journal of the RAS of Canada}
\newcommand{\memras}{Memoirs of the RAS}
\newcommand{\mnras}{Monthly Notices of the RAS}
\newcommand{\na}{New Astronomy}
\newcommand{\nar}{New Astronomy Review}
\newcommand{\pra}{Physical Review A: General Physics}
\newcommand{\prb}{Physical Review B: Solid State}
\newcommand{\prc}{Physical Review C}
\newcommand{\prd}{Physical Review D}
\newcommand{\pre}{Physical Review E}
\newcommand{\prl}{Physical Review Letters}
\newcommand{\pasa}{Publications of the Astron. Soc. of Australia}
\newcommand{\pasp}{Publications of the ASP}
\newcommand{\pasj}{Publications of the ASJ}
\newcommand{\rmxaa}{Revista Mexicana de Astronomia y Astrofisica}
\newcommand{\qjras}{Quarterly Journal of the RAS}
\newcommand{\skytel}{Sky and Telescope}
\newcommand{\solphys}{Solar Physics}
\newcommand{\sovast}{Soviet Astronomy}
\newcommand{\ssr}{Space Science Reviews}
\newcommand{\zap}{Zeitschrift fuer Astrophysik}
\newcommand{\nat}{Nature}
\newcommand{\iaucirc}{IAU Cirulars}
\newcommand{\aplett}{Astrophysics Letters}
\newcommand{\apspr}{Astrophysics Space Physics Research}
\newcommand{\bain}{Bulletin Astronomical Institute of the Netherlands}
\newcommand{\fcp}{Fundamental Cosmic Physics}
\newcommand{\gca}{Geochimica Cosmochimica Acta}
\newcommand{\grl}{Geophysics Research Letters}
\newcommand{\jcp}{Journal of Chemical Physics}
\newcommand{\jgr}{Journal of Geophysics Research}
\newcommand{\jqsrt}{Journal of Quantitiative Spectroscopy and Radiative Transfer}
\newcommand{\memsai}{Mem. Societa Astronomica Italiana}
\newcommand{\nphysa}{Nuclear Physics A}
\newcommand{\physrep}{Physics Reports}
\newcommand{\physscr}{Physica Scripta}
\newcommand{\planss}{Planetary Space Science}
\newcommand{\procspie}{Proceedings of the SPIE}

